CypherBench: Towards Precise Retrieval over Full-scale Modern Knowledge Graphs in the LLM Era

Retrieval from graph data is crucial for augmenting large language models (LLM) with both open-domain knowledge and private enterprise data, and it is also a key component in the recent GraphRAG system (edge et al., 2024). Despite decades of research on knowledge graphs and knowledge base question answering, leading LLM frameworks (e.g. Langchain and LlamaIndex) have only minimal support for retrieval from modern encyclopedic knowledge graphs like Wikidata. In this paper, we analyze the root cause and suggest that modern RDF knowledge graphs (e.g. Wikidata, Freebase) are less efficient for LLMs due to overly large schemas that far exceed the typical LLM context window, use of resource identifiers, overlapping relation types and lack of normalization. As a solution, we propose property graph views on top of the underlying RDF graph that can be efficiently queried by LLMs using Cypher. We instantiated this idea on Wikidata and introduced CypherBench, the first benchmark with 11 large-scale, multi-domain property graphs with 7.8 million entities and over 10,000 questions. To achieve this, we tackled several key challenges, including developing an RDF-to-property graph conversion engine, creating a systematic pipeline for text-to-Cypher task generation, and designing new evaluation metrics.

==> src/sec1-intro-alter.tex <==
\section{Introduction}

\begin{itemize}
    \item what
\end{itemize}


% Retrieval from graph data is crucial for augmenting large language models (LLM) with both open-domain relational knowledge and private enterprise data. Despite decades of research on knowledge graphs and knowledge base question answering (KBQA), leading LLM frameworks (\eg Langchain and LlamaIndex) have not yet supported retrieval from large-scale knowledge graphs like Wikidata. In contrast, retrieval from SQL databases has seen significant success, as demonstrated by numerous text-to-SQL research benchmarks dominated by LLM-based methods as well as widespread support in LLM frameworks. In this paper, we analyze the root cause of this discrepancy and suggest that traditional holistic RDF/SPARQL-based knowledge graphs (\eg Wikidata, Freebase) are less efficient for LLMs due to 1) overly large schemas that far exceed the typical LLM context window, 2) redundant and sometimes ambiguous relation types, 3) lack of type constraints on both entities and literal values, and 4) use of resource identifiers. As a solution, we propose shifting from holistic RDF graphs to multiple smaller property graphs, with \textit{Cypher} as the query language. This approach offers much greater prompt efficiency and human readability in the era of LLMs. We take the first step towards \textit{precise retrieval over large-scale graph databases} by introducing \textit{Cypherbench}, the first benchmark featuring 11 large-scale, multi-domain property graphs with 7.8 million entities and over 10,000 text-to-Cypher instances. We also address key technical challenges of large-scale text-to-Cypher, including baseline implementations and new evaluation metrics. Experimental results show that even template-generated Cypher queries present significant challenges for state-of-the-art LLMs such as GPT-4 and Claude 3. Beyond the benchmark, we also provide a comprehensive set of tools to support related research, including RDF-to-property-graph conversion, graph deployment dockers, automatic benchmark generation, visualization, and other resources.

% Over the past two years, large language models (LLMs) have demonstrated remarkable reasoning abilities across a wide range of tasks. 

% Large language models (LLMs) often struggle with knowledge-intensive tasks involving less popular entities \cite{}, latest events or private enterprise data \cite{}. Consequently, they usually require retrieval-augmented generation (RAG), which introduces an information retrieval step before prompting the LLM to generate an answer.

% The difficulty of this retrieval step, however, depends on the type of data being retrieved. Standard RAG methods based on top-$k$ embedding similarity have proven effective for large-scale text corpora. Similarly, retrieval from relational databases using text-to-SQL translation has also seen significant success with recent advancements in SQL generation capabilities in LLMs. The case for graph data, however, is different. Despite decades of research on knowledge graphs and knowledge base question answering (KBQA), leading LLM frameworks (\eg LangChain and LlamaIndex) has not yet supported retrieval from large-scale real world knowledge graphs like Wikidata as of the writing of this paper.

% Graphs, as a natural modality for modeling entity-relation data, have been widely adopted in both large-scale encyclopedic knowledge graphs like Wikidata and the storage of domain-specific enterprise data. Compared to raw textual documents, graphs enable efficient processing of complex aggregation\yanlin{clarify multi-hop vs. global queries somewhere in the paper} \saj{aggregation mitght not be the most impactful argument for graphs. Property graphs are definitely more suitable fot that. One possible approach can be to start with property graphs right off the bat} queries (\eg \textit{What is the average height of point guards who have played for the Toronto Raptors?}), where the answer might depend on information spread across thousands of documents or even the entire corpus. Graphs also provide a more compact representation of knowledge. For example, Wikidata contains on average 4.6 times the entities covered by Wikipedia across the domains we experimented with. These advantages has motivated decades of research in knowledge graphs and KBQA \cite{berant-etal-2013-semantic,moon-etal-2019-opendialkg,dubey2019lc,gu2021beyond,cao-etal-2022-kqa}, as well as the recent proposal of GraphRAG \cite{edge2024local,peng2024graph}.


\saj{what is the problem?} Large Language Models (LLMs) have demonstrated remarkable capabilities in natural language understanding, yet they are prone to hallucinations, particularly in knowledge-intensive tasks~\cite{petroni2021kilt} that require accurate, domain-specific, and up-to-date information. Addressing this challenge has led to a growing focus on augmenting LLMs with external information sources, such as knowledge graphs~\cite{todo:}, relational databases~\cite{todo:tag}, and the world wide web~\cite{todo:msft_llm_rag}. 
To this end, retrieval-augmented generation (RAG) have gained prominence, as the approach enables LLMs to incorporate verifiable external knowledge, thereby improving the accuracy and reliability of the generated output~\cite{todo:rationalizer}. \saj{play up the importance of KGs for RAG beyond web or wiki and the role of representation of KGs}

For relational databases, the retrieval step in RAG leverages SQL queries --- often generated using text-to-SQL methods~\cite{todo:text-2-sql} --- to obtain precise information related to a knowledge intensive task. However, such precise retrieval from large-scale knowledge graphs (\eg Wikidata~\cite{todo:wikidata}) to enhance LLMs via RAG remains a challenging problem due the absence of standardization in terms of the choice of the graph data model and retrieval protocol as well as lack of practical considerations such as retriever scalability, LLM's context limitations, and knowledge intensive task complexity.      
 

\saj{what is the problem? contd.} Previous studies on Knowledge Base Question Answering (KBQA), typically focused on simplified settings for evaluating algorithmic improvements (\saj{\eg ?}), smaller RDF graphs \cite{cao-etal-2022-kqa,baek-etal-2023-direct,emonet2024llm}. 
Moreover, we argue in \autoref{sec:rdf-to-property} the RDF representation is not amenable to the RAG setting, specifically for knowledge intensive tasks due to 

less difficult knowledge intensive tasks~\cite{berant-etal-2013-semantic,dubey2019lc,nie-etal-2022-graphq,baek-etal-2023-direct}, or impractical assumptions\cite{furrer2020compositional,kovriguina2023sparqlgen,banerjee2022modern} such 
%, which limits their practical application in real-world scenarios. 
As a result, leading LLM frameworks, including LangChain\footnote{\url{https://www.langchain.com/}} and LlamaIndex\footnote{\url{https://www.llamaindex.ai/}}, have only minimal support for retrieval from traditional RDF knowledge graphs like Wikidata as of the writing of this paper. Instead, they have prioritized retrieval from \textit{property graphs}, which are typically domain-specific with smaller schemas, using text-to-Cypher generation.

\saj{insert a figure motivating the KG-based RAG retreival. introduce text-to-query/cypher also.}

We analyze the root cause of why retrieval from traditional RDF knowledge graphs is challenging in \autoref{sec:rdf-to-property} and propose transforming the RDF graph into multiple smaller property graphs. These property graphs function as domain-specific \textit{views} (analogous to views in SQL databases) that can be efficiently queried by LLMs. This approach not only simplifies retrieval from traditional RDF knowledge graphs, but also enables the use of Cypher as a unified query language for both RDF graphs and property graph databases like Neo4j that are widely used in enterprise.

As a proof of concept, we introduced \textbf{Cypherbench}, a collection of 11 property graph databases transformed from Wikidata (detailed in \autoref{sec:graph}). Each graph contains the \textit{complete} set of entities and relations from Wikidata that conform to a domain-specific schema. Together, these graphs include a total of 7 million entities, covering roughly 25\% of Wikipedia and 6\% of Wikidata.  Along with the graph databases, we constructed over 10,000 natural language questions that spans 12 types of graph reasoning patterns (detailed in \autoref{sec:benchmark})~\saj{why are we focusing on graph reasoning patterns? we have to also define graph reasoning patterns.}. Notably, we include \textit{global queries} (defined as queries without any named entities), which have been largely overlooked by prior KBQA benchmarks. \yanlin{mention experiment results}.

In summary, this paper makes the following main contributions: \yanlin{mention the novelties in the techniques used}
\begin{itemize}[left=10pt]
    \item A proposal to use property graphs \saj{why is it large-scale?} and Cypher as a unified interface for graph retrieval, including both traditional RDF knowledge graphs and property graph databases like Neo4j.
    \item A collection of 11 large-scale \saj{}why is it large-scale? property graphs with 7 million entities, serving as groundwork for future property-graph-related research and as a high-quality locally-deployable knowledge source (with a knowledge cutoff of April 2024) for augmenting LLMs.
    \item An RDF-to-property-graph transformation engine for Wikidata that creates the aforementioned graphs, handling triple transformation, datatype conversion, and unit standardization.
    \item A text-to-Cypher / KBQA benchmark with over 10,000 instances spanning 12 types of graph patterns, covering global queries, temporal queries and complex aggregations.
    \item An automatic pipeline that generates text-to-Cypher tasks for any Neo4j graph database endpoint, used to create the aforementioned benchmark.
    % \item An automatic template-based text-to-Cypher task generation pipeline that creates the aforementioned benchmark, supports custom templates and works for any Neo4j graph database.
    \item A set of related tools, including graph deployment Docker containers, evaluation scripts, and graph visualization tools.
\end{itemize}


==> src/sec2-rdf-to-property-old.tex <==
\input{tables/graph_patterns}

\input{tables/return_patterns}

\input{tables/question_stats}


\section{From RDF to Property Graphs} \label{sec:rdf-to-property}

\begin{itemize}
    \item play up the importance of KGs for RAG beyond web or wiki and the role of representation of KGs
\end{itemize}

\subsection{Preliminaries: RDF and property graphs} \label{subsec:preliminary}

The Resource Description Framework (RDF) and property graph are two approaches to modeling and querying graph data. We begin with an abstract definition of a knowledge graph and then discuss how it is implemented in RDF and property graphs.

In its most basic form, a knowledge graph is a list of relations (or triples) in the format (subject entity, relation type, object entity), such as ("LeBron James", \texttt{playsFor}, "LA Lakers")\footnote{Relation types are also called properties in Wikidata or predicates in KBQA literature. In this paper, we use "properties" specifically to denote entity and relation attributes in property graphs.}. Additionally, entities are often assigned entity types (e.g., \texttt{Person}). Entities and relations can also be associated with literal values as properties (\eg \texttt{Player.height}, \texttt{receivesAward.year}).

The most popular public knowledge graphs to date (\eg Wikidata, Freebase, and DBpedia) are predominantly based on the RDF and queried using SPARQL. In RDF, entities are stored and accessed using Internationalized Resource Identifiers (IRIs). Entity properties, including entity names, are stored as relations, with the subject being the entity IRI and the object being a literal value. To store relation properties, RDF uses a process called reification, which creates a copy of the relation as a special entity\footnote{In Wikidata, this is referred to as a statement node. In Freebase, it is called a CVT node.}  and links it to the relation property using an additional relation.

\yanlin{Mention other usage of Neo4j, mention datahub} Property graph databases have gained significant popularity in industry in recent years, with Neo4j being the most popular graph database management system today\footnote{According to \url{https://db-engines.com/en/ranking/graph+dbms}}. Unlike RDF, the property graph model treats entities and relations as objects, each of which can be assigned types and have associated properties. In property graphs, entities are often accessed directly using their names. In this work, we adopt Neo4j and its query language, Cypher, as our property graph database system because of its popularity and strong community support. \saj{why property graph is chosen is not justified.}

\subsection{Why is Knowledge Graph Retrieval Hard?}

Retrieval over modern encyclopedic knowledge graphs, which are predominantly based on RDF/SPARQL, presents significant challenges for several reasons. Here, we use Wikidata as an example—the largest and most widely used knowledge graph today, containing 114 million entities and receiving 270 million edits contributed by over 12,000 active editors in the past year\footnote{\url{https://stats.wikimedia.org/\#/wikidata.org}}:
\begin{itemize}[left=10pt]
    \item \textit{Overly large schemas.}~~Encyclopedic knowledge graphs aim to cover entities and relations across all domains within a single graph, resulting in an extremely large schema that far exceeds the context window sizes of typical LLMs. For instance, Wikidata currently includes over 4 million entity types and 12,000 relation types. Furthermore, RDF graphs allow entities of arbitrary type to serve as subjects or objects for the same relation types, which further increases the number of unique relation schemas. \saj{a counter-argument to this might be to just extract relevant subgraphs and then put in the LLM context?}
    \item \textit{Use of resource identifiers.}~~ \saj{this is actually the schema linking and data awareness challenge.} The Wikidata SPARQL equivilant for question ``$Q4.$ What are the names of taxa that feed on Synsphyronus lathrius?'' in \autoref{tab:graph_patterns} is shown below, along with the annotated Cypher query in our proposed benchmark:\newline
    \begin{minipage}[t]{0.47\textwidth}
    \vspace{-5pt}
        \begin{tcolorbox}[title={\scriptsize SPARQL}, boxrule=0.8pt, colframe=gray, boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
            \begin{lstlisting}[style=TinyCypher]
SELECT ?name WHERE {
  item wdt:P31/wdt:P279* wd:Q16521.
  ?item wdt:P1034 wd:Q10687580.
  ?item rdfs:label ?name. FILTER(LANG(?itemLabel) = "en")
}
\end{lstlisting}
        \end{tcolorbox}
    \end{minipage}\hspace{0.01\textwidth}
    \begin{minipage}[t]{0.47\textwidth}
    \vspace{-5pt}
        \begin{tcolorbox}[title={\scriptsize Cypher}, boxrule=0.8pt, colframe=gray, boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
            \begin{lstlisting}[style=TinyCypher]
MATCH (n:Taxon)-[r0:feedsOn]->(m0:Taxon {name: 'Synsphyronus lathrius'})
RETURN n.name
\end{lstlisting}
        \end{tcolorbox}
    \end{minipage} 
    
    The SPARQL query contains identifiers for entities, entity types, relation types which must be obtained via external linkers \cite{sakor2020falcon,feng-etal-2023-calibrated} without forcing LLMs to memorize identifiers\yanlin{mention Cypher has better readability}.
    \item \textit{Overlapping and ambiguous relation types.}~~ Wikidata contains semantically overlapping relation types that are created for different domains and often used inconsistently. For instance, there are at least six relation types to indicate the starting time of an entity: {\small \texttt{start time (P580)}, \texttt{inception (P571)}, \texttt{date of official opening (P1619)}, \texttt{date of first performance (P1191)}, \texttt{publication date (P577)}, \texttt{service entry (P729)}}. This leads to considerable confusion when selecting the correct relation type to use during retrieval. \saj{this seems like schema ambiguity resulting from redundancy. but this doesn't seem like a general issue to KGs rather an artifact of the KG developer.}
    \item \textit{Lack of type constraints and normalization\yanlin{replace with unit standardization, change mentions in other places as well}.}~~RDF does not enforce type constraints and unit normalization on literal values of the same property. As a result, literal values in Wikidata often appear with different units and sometimes incorrect types, which leads to incorrect results when computing aggregation queries over these values. \saj{this is a great angle. we can borrow from text-to-SQL literature so show how adding schema and type improve generation of precise queries.}
\end{itemize}


\subsection{Hasn't KBQA already solved it?}

KBQA shares a similar goal of retrieving relevant information from a graph to answer questions. However, most existing studies focused on simplified settings to evaluate algorithmic improvements. For example, a common simplification made by recent work is assuming that the entity and relation identifiers are already provided \cite{furrer2020compositional,kovriguina2023sparqlgen,banerjee2022modern,luoreasoning,yu2022decaf}, which reduces the task to retrieval and reasoning over a small local subgraph. \saj{this is nice. basically this is the same as previous text-to-SQL method which assumes that the schema is known which is not practical. with this assumption they eliminate the need to do schema matching which is a limitation.} Moreover, many studies use custom-designed intermediate logical forms that lack support for certain graph querying functionalities (\eg relation properties querying\yanlin{Verify if relation properties are supported}, grouping, variable-length path matching) \cite{berant-etal-2013-semantic,berant-liang-2014-semantic,gu2021beyond,yih-etal-2015-semantic,cao-etal-2022-kqa,nie-etal-2022-graphq,li-etal-2023-shot}. \saj{didn't completely get this part. would be good to show with an example.} As a result, the majority of existing KBQA approaches (see \autoref{sec:related} for a complete categorization) struggle with some or all of the following types of queries: (1) queries involving relation properties, such as time-sensitive queries; (2) global queries that do not contain any named entities; and (3) queries requiring complex aggregations over a large number of entities. \saj{a great addition will be examples of such queries.}


% Despite a long history of research efforts in KBQA (detailed in \autoref{sec:related}), previous studies typically focused on simplified settings, using either smaller subgraphs \cite{cao-etal-2022-kqa,baek-etal-2023-direct,emonet2024llm}, simple queries without complex aggregation like grouping \cite{berant-etal-2013-semantic,dubey2019lc,nie-etal-2022-graphq,baek-etal-2023-direct}, or ignoring the identifiers \cite{furrer2020compositional,kovriguina2023sparqlgen,banerjee2022modern}, which limits their practical application in real-world scenarios. 

\subsection{Our Proposal: Property Graphs as a Unified Interface}

To address the aforementioned challenges, we propose transforming the holistic RDF graph into multiple domain-specific \textit{property graphs} and using Noe4j Cypher, the most popular graph query language today, as a unified query interface. These property graphs function as (materialized) \textit{views} on top of the original RDF graph, containing all data that conforms to their respective schemas and can be updated when the underlying RDF data changes (as illustrated in \autoref{fig:arch}).

This design enables scaling to a large number of domains without creating an overly complex schema, and eliminates ambiguity from overlapping relation types as they are now contextualized within specific domains. Our RDF-to-property-graph transformation layer manages datatype conversion and unit standardization, producing schema-enforced, strictly typed data that ensures the correctness for complex aggregation queries.

\saj{we can frame the entire section as justifying the property graphs as an important representation of KGs for RAG workflows. then we can additionally say, we introduce affordances to extend property graphs to RDFs --> it can be an HITL interface where we have automated and user-provided mechanisms to handle RDF to Cypher translation. To me this translation doesn't seem as straightforward as relation names may need standardization.}

\yanlin{Mention the questions benchmark}


==> src/sec3-graph-old.tex <==




\section{Transforming Wikidata into Property Graphs} \label{sec:graph}

\saj{We should generalize this to RDF to PGs. We can say in this paper we use wikidata as a case study due to size and popularity. }

\yanlin{Overview subsection? compare with previous RDF-to-property-graph conversion efforst. mention ours do not process raw RDF dump. Relate to the concept of view in databse}

% \subsection{Overview}

% This section describes our process for transforming Wikidata into property graphs. At a high level, we start by selecting a domain and manually curating the property graph schema, along with the mapping from the Wikidata schema to this schema. Next, our RDF-to-property-graph transformation engine uses the mapping to automatically construct a property graph by issuing SPARQL queries to the Wikidata endpoint. The property graph is stored in a DBMS-independent JSON format and is ultimately loaded into Neo4j.

\subsection{Schema Curation}

\yanlin{Discuss mapping triples to properties or relations}

\saj{since this might be KG specific such as Wikidata, DBpedia, Freebase, it would be great to sell it as a human-in-the loop solution with some design considerations. I can elaborate more in our meeting.}

We begin by selecting a domain and manually curating the property graph schema, along with the mapping from the Wikidata schema to this schema. This process typically involves identifying the entity and relation types and their properties relevant to the domain, followed by exploring Wikidata to find the corresponding Wikidata identifiers (QIDs for entity types and PIDs for relation types and properties). These information are stored in a JSON file that serves as input to the transformation engine. Sample entries in the JSON file are shown below:

\begin{minipage}[t]{0.47\textwidth}
    \vspace{-5pt}
        \begin{tcolorbox}[title={\scriptsize Sample Entity Schema with Wikidata Mappings}, boxrule=0.8pt, colframe=gray, boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
            \begin{lstlisting}[style=TinyJSON]
{
  "label": "Movie",
  "wd_source": "Q11424",
  "properties": [
    {
      "label": "runtime_minute",
      "wd_source": "P2047",
      "datatype": "float",
      "quantity_unit": "minute",
      "quantity_convert_unit": true
    }
  ]
}
\end{lstlisting}
        \end{tcolorbox}
    \end{minipage}\hspace{0.01\textwidth}
    \begin{minipage}[t]{0.47\textwidth}
    \vspace{-5pt}
        \begin{tcolorbox}[title={\scriptsize Sample Relation Schema with Wikidata Mappings}, boxrule=0.8pt, colframe=gray, boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
            \begin{lstlisting}[style=TinyJSON]
{
  "label": "receivesAward",
  "wd_source": "P166",
  "subj_label": "Movie",
  "obj_label": "Award",
  "properties": [
    {
      "label": "year",
      "wd_source": "P585",
      "datatype": "int"
    }
  ]
}
\end{lstlisting}
        \end{tcolorbox}
    \end{minipage} 

Each property is assigned a datatype. Properties that represent quantities are also given a unit, which is indicated in the property label (e.g., \texttt{runtime\_minute}) to inform LLMs during graph retrieval.

The authors created all 11 property graph schemas from scratch, with an average time investment of approximately 4 hours per graph.  The complete schema of a sample graph is presented in \autoref{tab:sample_graph}, and the schemas for all graphs are listed in \autoref{tab:all_graphs}.

\input{tables/sample_graph}

\subsection{Automatic RDF-to-property-graph Transformation}

\saj{how are we different from GraphQ-IR~\cite{nie-etal-2022-graphq}?}

\saj{also we should have some discussion on selecting Wikidata over DBpedia or other candidates.}

Next, our RDF-to-property-graph engine issues SPARQL queries to the Wikidata endpoint, using the identifiers from the graph schema file to fetch all entities and relations that conform to the specified schema. For example, the following SPARQL query (simplified for illustration) fetches all non-deprecated Wikidata \texttt{award received (P166)} relations where the subject is an instance of \texttt{Film (Q11424)} and the object is an instance of \texttt{Award (Q618779)}. These relations are then mapped to \texttt{receivesAward} relations in the target property graph.

\begin{minipage}[t]{\textwidth}
\vspace{-5pt}
    \begin{tcolorbox}[title={\scriptsize Wikidata SPARQL}, boxrule=0.8pt, colframe=gray, boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
        \begin{lstlisting}[style=TinyCypher]
SELECT DISTINCT ?subj ?obj ?statement
WHERE {
  ?subj wdt:P31 wd:Q11424. ?obj wdt:P31 wd:Q618779. ?subj p:P166 ?statement.
  ?statement ps:P166 ?obj. ?statement wikibase:rank ?rank. FILTER(?rank != wikibase:DeprecatedRank)
}
\end{lstlisting}
    \end{tcolorbox}
\end{minipage} 

The actual conversion engine is slightly more sophisticated, incorporating the following functionalities:

\begin{itemize}[left=10pt]
    \item \textit{Datatype conversion.} The engine enforces type constraints on property values by converting them into one of the following types and discarding those that cannot be converted: \texttt{str}, \texttt{int}, \texttt{float}, \texttt{date}, \texttt{list[str]}.
    \item \textit{Date conversion.} Wikidata stores precision for time values ranging from seconds up to centuries or more (\eg a historical event might be recorded with century-level precision like 18th century). For date properties, we retrieve the precision using the predicate \texttt{wikibase:timePrecision} and keep only those with a precision at least as fine as a date, which are ultimately mapped to Neo4j's \texttt{Date} values.
     \saj{this can go under Datatype conversion?}
     
    \item \textit{Unit standardization.} The engine enforces standardized units (\eg centimeters) on property values that represent quantities by converting all values that can be converted. This eliminates the need for unit conversion during retrieval and ensures accuracy of aggregation queries.  \saj{can this be a general step not only for wikidata but other DBs?}
    
    \item \textit{Rank filtering and time-sensitivity.} Wikidata uses rank to indicate the reliability or recency of a relation, which can be one of three values: preferred, normal, or deprecated. For time-sensitive relations (\eg the president of the United States), the currently valid entries are typically marked as preferred, while previously valid entries are marked as normal with additional properties indicating the relevant time period. For time-sensitive relations with time qualifiers in the target schema, we fetch all Wikidata relations with non-deprecated ranks, along with their starting and ending times. For other types of relations, we fetch only the highest-ranked available relation. \saj{can this be a general step not only for wikidata but other DBs?}
    
    \item \textit{Selective entity fetching.} The engine supports fetching only entities linked to certain relations to avoid out-of-memory issues for very broad entity types (e.g., people or organizations). For instance, in the movie graph, instead of fetching all instances of \texttt{Person} from Wikidata, the engine limits the fetch to only those connected to a \texttt{Movie} through relations like \texttt{directedBy} or \texttt{hasCastMember}. \saj{how is this enforcement done? this also seems like a design decision. Since our focus is on precise retrieval, we discard generic entity types to avoid augmenting LLMs with generic knowledge.}
    
\end{itemize}


The SPARQL queries issued by the engine are executed against a local Wikidata endpoint using the April 2024 Wikidata dump, allowing us to bypass the time limit of the official endpoint, and the results are aggregated into a schema-enforced strongly typed property graph. The transformation time ranges from seconds to hours, depending on the graph size. The graph statistics are shown in \autoref{tab:graph_stats}.

\input{tables/graph_stats}

\subsection{Neo4j Deployment} \label{subsec:neo4j_deployment}

The property graph is stored in a DBMS-independent JSON format and ultimately deployed using a custom Neo4j Docker container that initializes the data from the JSON file upon startup.

\saj{would be nice to show the entire process using a figure.}


==> tables/deprecated.tex <==
\begin{table*}[t]
\scriptsize
\begin{adjustwidth}{-1in}{-1in}
\centering
\begin{tabular}{llllllc}
\toprule
\textbf{Benchmark} & \textbf{Query Language} & \textbf{Data Model} & \textbf{Data Source} & \textbf{Schema Complexity} {\tiny (per db/graph)} & \textbf{Data Size} & \textbf{Zero-shot LLM?} \\
\midrule
Spider \cite{yu-etal-2018-spider} & SQL & relational data & Wikipedia and open tables & 27.6 columns & 400k rows & \checkmark \\
BIRD-SQL \cite{li2024can} & SQL & relational data & Kaggle and other open tables & 54.2 columns & 52M rows & \checkmark \\
LC-Quad 2.0 \cite{dubey2019lc} & SPARQL & RDF triples & Wikidata & 12k relation types & 100M entities & \texttimes \\
GrailQA \cite{gu2021beyond} & SPARQL & RDF triples & Freebase & 37k relation types & 45M entities & \texttimes \\
KQA Pro \cite{cao-etal-2022-kqa} & SPARQL, KoPL & RDF triples & Freebase subset & 0.8k relation types & 16k entities & \texttimes \\
MetaQA-Cypher \cite{nie-etal-2022-graphq} & Cypher & property graph & Open Movie Database & 5 relation types, 5 properties & 43k entities & \checkmark \\
Ours & Cypher & property graph & Wikidata & 7.5 relation types, 18.7 properties & 7M entities & \checkmark \\
\bottomrule
\end{tabular}
\end{adjustwidth}
\caption{Comparison of text-to-query benchmarks. The column ``Zero-shot LLM?'' refers to whether the benchmark is applicable to zero-shot evaluation by prompting LLM. Existing KGQA benchmarks are difficult to solve by prompting LLM in zero-shot scenarios due to the massive schema of traditional RDF-based knowledge graphs.}
\label{tab:nl2q_overview}
\end{table*}

